GOAT-Bench: A Benchmark for Multi-Modal Lifelong Navigation

The Embodied AI community has made significant strides in visual navigation tasks, exploring targets from 3D coordinates, objects, language descriptions, and images. However, these navigation models often handle only a single input modality as the target. With the progress achieved so far, it is time to move towards universal navigation models capable of handling various goal types, enabling more effective user interaction with robots. To facilitate this goal, we propose GOAT-Bench, a benchmark for the universal navigation task referred to as GO to AnyThing (GOAT). In this task, the agent is directed to navigate to a sequence of targets specified by the category name, language description, or image in an open-vocabulary fashion. We benchmark monolithic RL and modular methods on the GOAT task, analyzing their performance across modalities, the role of explicit and implicit scene memories, their robustness to noise in goal specifications, and the impact of memory in lifelong scenarios.

==> fig/teaser.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
% \vspace{-0.5cm}
\captionsetup{type=figure}
\includegraphics[width=\linewidth]{fig/teaser-updated-new.png}
\captionof{figure}{We study the Go to Any Thing (GOAT) task, which involves agents navigating to a sequence of open vocabulary goals specified through any of the three modalities – category name, a language description, or an image.
We propose GOAT-Bench, a benchmark for the GOAT task, where we evaluate modular and monolithic, explicit and implicit map-based navigation approaches.
In the above example, we task the agent with sequentially navigating to 1) a recliner chair (from a closed set of \textit{k} categories), 2) the oven shown in the picture, 3) \myquote{the white book on the coffee table in the living room}, and some other objects in the scene. The goal of the benchmark is to facilitate progress towards building such universal, multi-modal, lifelong agents. 
}
\label{fig:teaser}
\end{center}
}]

==> tables/fp_vs_pt_122.tex <==
\begin{table}
\centering
\begin{tabular}{@{} llcc @{}}
\toprule
Evaluation & Train dataset & Success $\uparrow$ & SPL $\uparrow$ \\
\midrule
\multirow{2}{*}{Zero-shot}
& ProcTHOR-122 & 13 \stderr{1.03} & 6 \stderr{0.51}  \\
& \ourdataset-122 & \best{19} \stderr{1.19} & \best{7} \stderr{0.48} \\
\midrule
\multirow{2}{*}{Fine-tuned}
& ProcTHOR-122 & 46 \stderr{1.52} & 21 \stderr{0.85} \\
& \ourdataset-122 & 46 \stderr{1.52} & \best{22} \stderr{0.86}\\
\bottomrule
\end{tabular}
\caption{
\textbf{Performance of agents trained on scale-matched \ourdataset and ProcTHOR and evaluated on HM3DSem.}
We compare agents trained on \ourdataset and a scale-matched set of 122 ProcTHOR scenes with and without finetuning.
With equal scene dataset sizes, \ourdataset leads to better agent performance in both zero-shot and fine-tuned settings.
The higher visual fidelity and correlation to HM3DSem of \ourdataset scenes are likely contributing to this improved performance.
}
\label{tab:fp_vs_pt-122}
\end{table}


==> tables/fps_benchmark.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}
{%
\begin{tabular}{@{} l rrr rrr @{}}
\toprule
 & \multicolumn{3}{c}{ProcTHOR-S (FPS $\uparrow$)} & \multicolumn{3}{c}{ProcTHOR-L (FPS $\uparrow$)} \\ %
\cmidrule(l{2pt}r{2pt}){2-4}
\cmidrule(l{2pt}r{0pt}){5-7}
Simulator & 1 Proc & 1 GPU & 8 GPU & 1 Proc & 1 GPU & 8 GPU \\
\midrule

AI2-THOR~\cite{kolve2017ai2} & \makecell{240\\{\footnotesize $\pm$69}} & \makecell{1,427\\{\footnotesize $\pm$74}} & \makecell{8,599\\{\footnotesize $\pm$359}} & \makecell{115\\{\footnotesize $\pm$19}} & \makecell{6,280$^\ast$\\{\footnotesize $\pm$40}} & \makecell{3,208\\{\footnotesize $\pm$127}} \\
\makecell[l]{Habitat~\cite{savva2019habitat,szot2021habitat}\\(uncompressed)} & \makecell{2,297\\{\footnotesize $\pm$447}} & \makecell{6,374\\{\footnotesize $\pm$798}} & \makecell{57,160\\{\footnotesize $\pm$4,917}} & \makecell{1,007\\{\footnotesize $\pm$187}} & \makecell{5,237\\{\footnotesize $\pm$1,130}} & \makecell{39,510$^\dagger$\\{\footnotesize $\pm$6,345}} \\

\makecell[l]{Habitat~\cite{savva2019habitat,szot2021habitat}\\(compressed)} & \makecell{\best{2,523}\\{\footnotesize $\pm$300}} & \makecell{\best{7,363}\\{\footnotesize $\pm$394}} & \makecell{\best{58,947}\\{\footnotesize $\pm$1,804}} & \makecell{\best{1,233}\\{\footnotesize $\pm$224}} & \makecell{\best{6,508}\\{\footnotesize $\pm$495}} & \makecell{\best{46,674}\\{\footnotesize $\pm$5,640}} \\

\bottomrule
\end{tabular}
}
\vspace{1pt}
\caption{
\textbf{Benchmark of navigation FPS.}
We optimize ProcTHOR scenes similarly to \ourdataset and compare performance when the assets are loaded in Habitat to the original scenes in AI2-THOR.
We observe close to an order of magnitude of improvement of simulation performance across most setups.
$^\ast$After correspondence with \citet{deitke2022procthor}, the authors confirmed this number is a typo and the true number is unknown.
$^\dagger$ProcTHOR-L 8-GPU benchmark conducted with 7 processes per GPU instead of 15 due to memory bottlenecks.
}
\label{tab:fps_benchmark}
\end{table}


